Guiding Enumerative Program Synthesis with Large Language Models

Pre-trained Large Language Models (LLMs) are beginning to dominate the discourse around automatic code generation with natural language specifications. In contrast, the best-performing synthesizers in the domain of formal synthesis with precise logical specifications are still based on enumerative algorithms. In this paper, we evaluate the abilities of LLMs to solve formal synthesis benchmarks by carefully crafting a library of prompts for the domain. When one-shot synthesis fails, we propose a novel enumerative synthesis algorithm, which integrates calls to an LLM into a weighted probabilistic search. This allows the synthesizer to provide the LLM with information about the progress of the enumerator, and the LLM to provide the enumerator with syntactic guidance in an iterative loop. We evaluate our techniques on benchmarks from the Syntax-Guided Synthesis (SyGuS) competition. We find that GPT-3.5 as a stand-alone tool for formal synthesis is easily outperformed by state-of-the-art formal synthesis algorithms, but our approach integrating the LLM into an enumerative synthesis algorithm shows significant performance gains over both the LLM and the enumerative synthesizer alone and the winning SyGuS competition tool.

==> temp.tex <==

% We tested different LLMs on randomly picked benchmarks with different prompts. Models and prompts are shown below.

% \section{Prompt Styles}
% There are two main prompt styles, the Currie models(with or without fine-tuned) use the first style, and the GPT4 uses the second style.

% \subsection{Prompt Style: 1}

% We construct prompts from each SyGuS benchmark that looks like the SMT verification problem and ask the LLM to complete the define-fun.

% This is the max benchmark:
% \begin{lstlisting}[language=smt, style=smt-style]
% (set-logic LIA)

% (synth-fun max2 ((x Int) (y Int)) Int))

% (declare-var x Int)
% (declare-var y Int)
% (constraint (>= (max2 x y) x))
% (constraint (>= (max2 x y) y))
% (constraint (or (= x (max2 x y)) (= y (max2 x y))))

% (check-synth)
% \end{lstlisting}

% This is the corresponding prompt:
% \begin{lstlisting}[language=smt, style=smt-style]
% (set-logic LIA)

% (declare-fun x () Int)
% (declare-fun y () Int)
% (assert (or (not (>= (max2 x y) x))
%          (not (>= (max2 x y) y))
%           (not (or (= x (max2 x y)) (= y (max2 x y))))))

% (check-sat)
% (define-fun max2 ((x Int) (y Int)) Int
% (
% \end{lstlisting}

% \subsection{Prompt style: 2}
% \begin{itemize}
%     \item Detect if the benchmark is a LIA\_INV problem, if so, generate the prompt for the LIA\_INV problem, otherwise, generate the prompt for the LIA problem.

%     \item LIA\_INV problem:
%         \begin{itemize}
%             \item Get the pre-condition, transition, and post-condition
%             \item Get the invariant constraint
%             \item Include pre-f, trans-f, post-f, and the inv-constraint to the prompt, and add a guided prompt to generate the Python method:
            
%                 1. Guide prompt 1: Explanation of the SMT-LIB code:
        
%                 2. Guide prompt 2: Write a Python method \{function name\} that meets the constraint requirement. The method should not contain any built-in method.
        
%                 3. Guide prompt 3: Translate the Python method into SMT-LIB code \{function name\} and only the SMT-LIB code.
%         \end{itemize}
%         \item LIA problem:
%             \begin{itemize}
%                 \item Include the declare-vars and constraints, and add a guided prompt to generate the Python method
%                 \item Guide prompt 1: Write a Python method {function name}.  Requirements: 1. No built-in Python functions. 2. Never violate the SMT-LIB constraints above.
%                 \item Guide prompt 2: Translate the Python method into SMT-LIB code {function name} and only the SMT-LIB code.
%             \end{itemize}
%         \item Each new prompt should contain the previous prompts and responses.
% \end{itemize}

% One of the LIA\_INV prompts' example:

% This is the fib\_01 benchmark
% \begin{lstlisting}[language=inv-smt, style=smt-style]
% (set-logic LIA)

% (synth-inv inv-f ((x Int) (y Int)))

% (define-fun pre-f ((x Int) (y Int)) Bool
%     (and (= x 1) (= y 1)))
% (define-fun trans-f ((x Int) (y Int) (x! Int) (y! Int)) Bool
%     (and (= x! (+ x y)) (= y! (+ x y))))
% (define-fun post-f ((x Int) (y Int)) Bool
%     (>= y 1))

% (inv-constraint inv-f pre-f trans-f post-f)

% (check-synth)
% \end{lstlisting}
% These are the corresponding prompts:

% \begin{lstlisting}[language=inv-smt, style=smt-style]
% (synth-inv inv-f ((x Int) (y Int)))

% (define-fun pre-f ((x Int) (y Int)) Bool
%     (and (= x 1) (= y 1)))
% (define-fun trans-f ((x Int) (y Int) (x! Int) (y! Int)) Bool
%     (and (= x! (+ x y)) (= y! (+ x y))))
% (define-fun post-f ((x Int) (y Int)) Bool
%     (>= y 1))

% (inv-constraint inv-f pre-f trans-f post-f)

% Explanation of the SMT-LIB code:
% \end{lstlisting}

% \begin{lstlisting}[language=inv-prompt, style=smt-style]
% ** Previous prompt and solution **

% Write only one Python method {inv_prompt} without 
% any built-in methods that meets the requirement of 
% the constraint. The method should not contain any 
% built-in method.

% \end{lstlisting}

% \begin{lstlisting}[language=inv-prompt, style=smt-style]
% ** Previous prompts and solutions **

% Translate the Python method into SMT-LIB code 
% {inv_prompt} and only the SMT-LIB code.

% \end{lstlisting}

% \texttt{inv\_prompt} is \texttt{inv-f((x Int) (y Int))} in this case, which contains the function name and variables.

% For other non-INV LIA benchmarks, we simply remove the first prompt and use the second and third directly.

% \section{Simple Prompts}

% \subsection{Curie with no fine-tuning}
% We tested the original Curie model with the 101 benchmarks(without LIA\_INV), CVC5 solved 3. 

% We remove the LIA\_INV, because the INV conditions are hard for Curie to understand, and Curie cannot provide useful solutions. In order to decrease the experiment time and the API usage, we didn't count the INVs.

% \subsection{Curie with fine-tuning}
% We fine-tuned the model with a training set containing 870 benchmarks. We also changed all the numerals into decimal digits and used \texttt{\textbackslash n;\#\#\#\textbackslash n} as the end mark of prompts, \texttt{\textbackslash n;END} for completions. For example:

% \begin{lstlisting}[language=smt, style=JSON]
%  {"prompt":" (set-logic BV)\n(declare-fun x  () (_ BitVec 32))\n(define-fun hd03 ((x (_ BitVec 32))) (_ BitVec 32)\n    (bvand x (bvneg x)))\n(assert (or (not (= (hd03 x) (f x)))))\n(check-sat)\n; define function f\n(define-fun f ((x (_ BitVec 32))) (_ BitVec 32)\n;###\n",
%  "completion":" (bvand x (bvneg x))) \n;END"}
% \end{lstlisting}

% We tested the fine-tuned Curie with the same 101 benchmarks testing set, Model solved 37.

% \subsubsection{Without Let Expression}

% We fine-tuned the previous fine-tuned Curie model with a new training set which expanded the let expressions. The results remain the same. 

% \subsubsection{Rename Function Names and Variables}
% The function names followed by define-fun are changed into ffX, where X is an index. The first define-fun function's name will be ff1. And each variable name also has been changed into vvX, where X is an index.

% We then fine-tuned Curie with renamed training set and tested the fine-tuned model. Model solved 24 over 101 testing benchmarks.

% \subsubsection{Another fine-tuned Curie}
% We then fine-tuned Curie twice with another 870 randomly selected benchmarks training set and tested on 333 benchmarks. The testing benchmarks' functions' and variables' names are changed. 

% One is fine-tuned with a pure training set without any let expression. CVC5 solved 36 over 333 benchmarks(BV, LIA, LIA\_INV). Another fine-tuning is with let expressions. Model solved 39 over 333 benchmarks. 

% If we tested with the benchmarks that didn't change the names, the LLM which solved 39 can solve 72. The total testing set is 332 because one of the original benchmarks’ variables and function names are too long to handle for LLM.


% \section{Complex Prompts}

% We also used Davinci and GPT-4 as the LLM with complex prompts. First, we detect if the benchmark is a LIA\_INV problem, if so, generate the prompt for the LIA\_INV problem, otherwise, create the prompt for the LIA problem. We haven't tested on BV benchmarks yet.

% We run prompts for each benchmark at most 4 times to get a result. If the LLM solved the benchmark, it stops, otherwise, it continuing generates new solutions for checking.

% We didn't fine-tune Davinci, because the fine-tuned model cannot provide useful explanations and correct Python codes. We randomly select 216 LIA benchmarks (containing INVs). Davinci solved 127 over 216 benchmarks.

% Using the same prompts, we tested GPT4 with the same benchmarks. It solved 134 benchmarks within 252 attempts. On average, GPT-4 takes 1.9 attempts to get a correct solution.

% In non-inv benchmarks, there are 2 benchmarks(max6, max12) cannot be translated correctlt form python to SMT-lib. 'max6' has a for loop. 18 benchmarks are failing because the original python it produces is semantically wrong. "example*", "guard*", "ite*" are failing because the GPT4 cannot handle too many define-funs. 2 benchmarks(max4, max7) are failing because the solution parser.

